InfoGAN-CR and ModelCentrality: Self-supervised Model Training and Selection for Disentangling GANs

Disentangled generative models map a latent code vector to a target space, while enforcing that a subset of the learned latent codes are interpretable and associated with distinct properties of the target distribution. Recent advances have been dominated by Variational AutoEncoder (VAE)-based methods, while training disentangled generative adversarial networks (GANs) remains challenging. In this work, we show that the dominant challenges facing disentangled GANs can be mitigated through the use of self-supervision. We make two main contributions: first, we design a novel approach for training disentangled GANs with self-supervision. We propose contrastive regularizer, which is inspired by a natural notion of disentanglement: latent traversal. This achieves higher disentanglement scores than state-of-the-art VAE- and GAN-based approaches. Second, we propose an unsupervised model selection scheme called ModelCentrality, which uses generated synthetic samples to compute the medoid (multi-dimensional generalization of median) of a collection of models. The current common practice of hyper-parameter tuning requires using ground-truths samples, each labelled with known perfect disentangled latent codes. As real datasets are not equipped with such labels, we propose an unsupervised model selection scheme and show that it finds a model close to the best one, for both VAEs and GANs. Combining contrastive regularization with ModelCentrality, we improve upon the state-of-the-art disentanglement scores significantly, without accessing the supervised data.

==> disentangling_analysis.tex <==
{\color{red}
\section{Disentangling in linear Gaussian generators under InfoGAN and CR regularizers}
\label{sec:disent_analysis}

{\bf Sewoong: can we prove Theorem 4 for any other divergence?  It is tricky as $\Sigma^{(i)}$'s are degenerate, i.e.~ Gaussians. with covariances that are not full rank. some directions have variance zero. I did some calculations, and because we have degenerate distributions, Pairwise KL and Pairwise Hellinger does not work. Pairwise JS gets complicated, and probably. does not give what. we want.}

{\bf Sewoong: IB-GAN (https://openreview.net/pdf?id=ryljV2A5KX) probably does not get PCA either. Can we prove it? and another theorem? } 

{\bf We might want to add experimental results using just CR (both with/without our model selection).}

\begin{assume} \label{assum:asssume1}
Suppose $\cN_{k}(\mu, \Sigma)$ denote a $k \in \naturals$ dimensional multivariate Gaussian random variable with mean $\mu \in \reals^k$ and covariance matrix $\Sigma \in \reals^{k \times k}$. 
Let the real samples be i.i.d.~with zero mean $d$-dimensional multivariate Gaussian distribution $\cN_{d}(0, \Sigma)$, with invertible covariance matrix $\Sigma \in \reals^{d \times d}$. 
Let $C \sim \cN_{r}(0, \id)$, and $Z \sim \cN_{d}(0, \id)$ be two latent random vectors of the generator, with multivariate zero mean Gaussian distribution with identity covariance matrices $\id \in \reals^{r \times r}$, and $\id \in \reals^{d \times d}$ respectively, with the additional constraint that $r \leq d$.
Let $\mathcal{G}$ be a class of linear generators, such that $\mathcal{G} = \{G:\reals^r \times \reals^d \to \reals^d \,|\, G(c, z) = Bc + Az,\,  B \in \reals^{d \times r},\, A \in \reals^{d \times d} \}$, parameterized by matrices $B$ and $A$, and let the generated random sample be denoted as $X = G(C, Z)$.
\end{assume}

\begin{theorem}
Suppose the Assumption~\ref{assum:asssume1} holds and $\mathcal{Q}$ be a class of factorized Gaussian conditional distributions in the space $C|X$, such that $\mathcal{Q} = \{Q \,|\, Q_{c|x} = (1/\sqrt{2\pi})^{r} \exp \{-(1/2)\|c - \mu(x)\|^2,\, \mu: \reals^d \to \reals^r\}$, parametrized by function $\mu(\cdot)$.

Then any generator $G \in \mathcal{G}$, which maximizes the InfoGAN regularizer~\eqref{eq:InfoGANloss}, $\max_{Q \in \cQ} \cL_{\rm Info}(G, Q)$, subject to the condition that the generated distribution is same as the real distribution, i.e.~$X = G(C,Z) \sim \cN_{d}(0, \Sigma)$, has the parameter $B = \Sigma^{1/2} U$, where $U \in \reals^{d \times r}$ is some semi-orthonormal matrix, i.e.~$U^T U  = \id_{r \times r}$.
\end{theorem}
\begin{proof}
We start our analysis by computing the InfoGAN regularizer for a fixed generator $G \in \mathcal{G}$, by re-writing the InfoGAN regularizer~\eqref{eq:InfoGANloss} as,
\begin{align}
\underset{Q \in \cQ}\max \, \cL_{\rm Info}(G, Q) &= \underset{Q \in \cQ}\max\, \E_{X, C}[\log Q_{c|X}(C)] \nonumber \\
&= \underset{\mu: \reals^d \to \reals^r}\max\, \E_{X, C}[\log ((1/\sqrt{2\pi})^{r} \exp \{-(1/2)\|C - \mu(X)\|^2) ] \nonumber \\
&= \E_{X}[\underset{\mu(X) \in \reals^r}\max\,  \E_{C|X} [-(1/2)\|C - \mu(X)\|^2 ]  - (r/2) \log (2 \pi) \nonumber \\
&= \E_{X}[\E_{C|X} [-(1/2)\|C - \E_{C|X} [C]\|^2 ] - (r/2) \log (2 \pi) \label{eq:infogan_loss_equiv}
\end{align}
where the last equality is true since $\E_{C|X} [C]$ minimizes the quadratic in $y$, $\E_{C|X} [\|C - y\|^2] = \E_{C|X} [\|C\|^2] -2\E_{C|X} [C] y + y^2$. Next we compute $\E_{C|x} [C]$ as follows. Since $X = G(C, Z) = BC + AZ$, is linear combination of independent Gaussian random variables $C$ and $Z$, $(C^T, X^T)^T$ is jointly Gaussian~\cite{hajek2015random} with zero mean and covariance matrix $\begin{bmatrix}
\Sigma_{CC^T} & \Sigma_{CX^T}\\
 \Sigma_{XC^T} & \Sigma_{XX^T}
\end{bmatrix} = \begin{bmatrix}
\id & B^T\\
B & \Sigma
\end{bmatrix}$, where we used the fact that $X \sim \cN_{d}(0, \Sigma)$ and $C \sim \cN_{r}(0, \id)$. This implies that, since $\Sigma$ is invertible, the conditional mean is given by 
\begin{align}\label{eq:infogan-conditional-mean}
\E_{C|x} [C] = \Sigma_{CX^T} \, \Sigma_{ XX^T}^{-1} \, x = B^T \Sigma^{-1} x \,.
\end{align}
Additionally, similar arguments also proves that
\begin{align}\label{eq:infogan-covariance}
\Sigma = \E_{X}[XX^T] &= \E_{C, Z}[(BC+AZ)(BC+AZ)^T] \nonumber \\
&= \E_{C}[B C C^T B^T]+ \E_{C, Z}[B C Z^T A^T + A Z C^T B^T] + \E_{Z}[A Z Z^T A^T]  \nonumber \\
&= B \id B^T + 0 + A \id A^T = BB^T + AA^T\,.
\end{align}
Now we are ready to characterize the minimizer of InfoGAN regularizer subject to $X = G(C,Z) \sim \cN_{d}(0, \Sigma)$ as follows. Using \ref{eq:infogan_loss_equiv}, this optimization problem is equivalent to
\begin{align}
\max_{\substack{{G \in \mathcal{G}} \\ {G(C,Z) \sim \cN_{d}(0, \Sigma)}}} \underset{Q \in \cQ}\max \; \cL_{\rm Info}(G, Q) &= \max_{\overset{G \in \mathcal{G}}{X = G(C,Z) \sim \cN_{d}(0, \Sigma)}} \E_{X}[\E_{C|X} [-(1/2)\|C - \E_{C|X} [C]\|^2 ] - (r/2) \log (2 \pi) \nonumber \\
 &= \max_{\substack{{G \in \mathcal{G}} \\ {X = G(C,Z) \sim \cN_{d}(0, \Sigma)}}}  -(1/2) \E_{X}[\E_{C|X} [\|C\|^2] - \| \E_{C|X} [C]\|^2 ] - (r/2) \log (2 \pi) \nonumber \\
 &= \max_{\substack{{G \in \mathcal{G}} \\ {X = G(C,Z) \sim \cN_{d}(0, \Sigma)}}} -(1/2) \E_{C}[\|C\|^2] + (1/2) \E_{X}[\| B^T \Sigma^{-1} X\|^2 ] - (r/2) \log (2 \pi) \nonumber \\
 &= \max_{\substack{{B \in \reals^{d \times r},\, A \in \reals^{d \times d}} \\ {BB^T + AA^T = \Sigma}}} \, (-r + \E_{X}[\| B^T \Sigma^{-1} X\|^2 ] - r \log (2 \pi))/2\,,\label{eq:infogan_loss_eq1}
\end{align}
where the third equality follows from \eqref{eq:infogan-conditional-mean} and the final equality follows from the definition of class $\mathcal{G}$, \eqref{eq:infogan-covariance}, and $C \sim \cN_r(0, \id)$.  We simplify the second term above as follow.
\begin{align}
\E_{X}[\| B^T \Sigma^{-1} X\|^2 ] &= \E_{C, Z}[\trace{ X^T \Sigma^{-1} B B^T \Sigma^{-1} X }] \nonumber \\&
= \E_{C, Z}[\trace{ \Sigma^{-1} B B^T \Sigma^{-1} XX^T } ] \nonumber \\&
= \trace{ \Sigma^{-1} B B^T \Sigma^{-1} \E_{C, Z}[XX^T ]} \nonumber \\&
= \trace{ \Sigma^{-1} B B^T \Sigma^{-1} \Sigma} \nonumber \\&
= \trace{ \Sigma^{-1} B B^T} = \trace{B^T \Sigma^{-1/2} \Sigma^{-1/2} B}
= \|\Sigma^{-1/2} B \|_F^2\label{eq:infogan_loss_eq2}
\end{align}
Substituting \eqref{eq:infogan_loss_eq2} into \eqref{eq:infogan_loss_eq1}, we get
\begin{align}
\max_{\substack{{G \in \mathcal{G}} \\ {G(C,Z) \sim \cN_{d}(0, \Sigma)}}} \underset{Q \in \cQ}\max \; \cL_{\rm Info}(G, Q) &= \max_{\substack{{B \in \reals^{d \times r},\, A \in \reals^{d \times d}} \\ {BB^T + AA^T = \Sigma}}} \, (1/2)\|\Sigma^{-1/2} B \|_F^2- (r/2) (1 + \log (2 \pi)) \nonumber \\
&= \max_{\substack{{B \in \reals^{d \times r}} \\ {BB^T \preccurlyeq \Sigma}}} \, (1/2) \|\Sigma^{-1/2} B \|_F^2- (r/2) (1 + \log (2 \pi)) \nonumber \\
&= \max_{\substack{{\tilde{B} \in \reals^{d \times r}} \\ {\tilde{B}\tilde{B}^T \preccurlyeq \id}}} \, (1/2) \|\tilde{B} \|_F^2- (r/2) (1 + \log (2 \pi)) \nonumber \\
&\leq r/2 - (r/2) (1 + \log (2 \pi)) =  (r/2) \log (2 \pi)\,,
\end{align}
where the third equality follows from setting $\tilde{B} = \Sigma^{-1/2} B$ and the second to last inequality follows from %
$\tilde{B}\tilde{B}^T \preccurlyeq \id$
and ${\rm rank}(B) = r$. By the existence of SVD of $\tilde{B}$, the upper-bound is achieved iff $\tilde{B}$ is any orthonormal matrix $U \in \reals^{d \times r}$ or equivalently iff $B = \Sigma^{1/2} U$
\end{proof}

\begin{theorem}
	Suppose the Assumption~\ref{assum:asssume1} holds. Let $\sum_{i=1}^d \sigma_i u_i u_i^T$ be the eigenvalue decomposition of the positive definite covariance matrix $\Sigma$, such that $ \sigma_1 > \sigma_2 > \ldots > \sigma_d > 0$ and $u_i^T u_j = \delta_{ij}$. Then, for $r > 1$, any generator $G \in \mathcal{G}$, which maximizes the following diveregence, 
	\begin{align}
		\frac1{4(r-1)} \sum_{\substack{i,j \in [r] \\ i \neq j}} \|\Sigma^{(i)} - \Sigma^{(j)}\|_F^2\,,
	\end{align}
	where $\Sigma^{(i)} = {\rm Cov}_{Q^{(i)}} ((X^T, X'^T)^T)$ is the covariance matrix corresponding to the joint distribution $Q^{(i)}$ of $(X^T,X'^T)^T$, as defined in Theorem~\ref{rem:js}, subject to the condition that the generated distribution is same as the real distribution, i.e.~$X = G(C,Z) \sim \cN_{d}(0, \Sigma)$, 
	has the parameter $B =\sum_{i=1}^r \sqrt{\sigma_i} u_{i} e_{\pi(i)}^T$, where $\pi:[r] \to [r]$ is some permutation of $(1,2,\ldots,r)$.
\end{theorem}
\begin{proof}
It is easy to check that the covariance matrix of distribution $Q^{(i)}$ is
\begin{align}
\Sigma^{(i)} = {\rm Cov}_{Q^{(i)}} ((X^T, X'^T)^T) = \begin{bmatrix}
\Sigma & b^{(i)}(b^{(i)})^T\\
b^{(i)}(b^{(i)})^T & \Sigma
\end{bmatrix}\,,
\end{align}
where $b^{(i)}$ denotes the $i$-th column of matrix $B$. Then we can simplify the sum of squared differences of the covariance matrices as
\begin{align}
\sum_{\substack{i,j \in [r] \\ i \neq j}} \|\Sigma^{(i)} - \Sigma^{(j)}\|_F^2 &= 2 \sum_{\substack{i,j \in [r] \\ i \neq j}} \|b^{(i)}(b^{(i)})^T - b^{(j)}(b^{(j)})^T\|_F^2 \nonumber \\
&= 2 \sum_{\substack{i,j \in [r] \\ i \neq j}} \Ip{b^{(i)}}{b^{(i)}}^2 + \Ip{b^{(j)}}{b^{(j)}}^2 - 2\Ip{b^{(i)}}{b^{(j)}}^2 \nonumber \\
&\leq 4(r-1) \sum_{\substack{i\in [r]}} \Ip{b^{(i)}}{b^{(i)}}^2 \nonumber \\
&\leq 4(r-1) \sum_{\substack{i,j \in [r]}} \Ip{b^{(i)}}{b^{(j)}}^2 \nonumber \\
&= 4(r-1) \|B^TB\|_F^2 \nonumber \\
&= 4(r-1) \|BB^T\|_F^2\,,
\end{align}
where we used $0 \leq \Ip{b^{(i)}}{b^{(j)}}^2$ when $i \neq j$. Now, using this and \eqref{eq:infogan-covariance}, we can show that,
\begin{align}
\max_{\substack{{G \in \mathcal{G}} \\ {X = G(C,Z) \sim \cN_{d}(0, \Sigma)}}} \frac1{4(r-1)} \sum_{\substack{i,j \in [r] \\ i \neq j}} \|\Sigma^{(i)} - \Sigma^{(j)}\|_F^2 &\leq \max_{\substack{{B \in \reals^{d \times r},\, A \in \reals^{d \times d}} \\ {BB^T + AA^T = \Sigma}}} \,  \|BB^T\|_F^2 = \max_{\substack{{B \in \reals^{d \times r}} \\ {BB^T \preccurlyeq \Sigma}}} \,  \|BB^T\|_F^2\,.
\end{align}

Next we will prove that $BB^T$ which maximizes the above objective, is the rank $r$ approximation, $\Sigma_r = \argmax_{\substack{ {\hat{\Sigma} \in \reals^{d \times d}} \\ {{\rm rank}(\hat{\Sigma}) = r} }} \|\Sigma - \hat{\Sigma} \|_F^2$, of $\Sigma$. Since $\sum_{i=1}^d \sigma_i u_i u_i^T$ is the eigenvalue decomposition of the positive definite covariance matrix $\Sigma$, such that $ \sigma_1 > \sigma_2 > \ldots > \sigma_d > 0$ and $u_i^T u_j = \delta_{ij}$, by Eckart–Young–Mirsky theorem $\Sigma_r = \sum_{i=1}^r \sigma_i u_i u_i^T$. Notice that 
$0 \preccurlyeq \Sigma_r = \sum_{i=1}^r \sigma_i u_i u_i^T \preccurlyeq \sum_{i=1}^d \sigma_i u_i u_i^T = \Sigma$
which gives the following,
\begin{align}
\|\Sigma - \Sigma_r \|_F^2 = \min_{\substack{ {\hat{\Sigma} \in \reals^{d \times d}} \\ {{\rm rank}(\hat{\Sigma}) = r} }} \|\Sigma - \hat{\Sigma}\|_F^2 %
&= \min_{\substack{ {\hat{\Sigma} \in \reals^{d \times d}} \\ {{\rm rank}(\hat{\Sigma}) = r} \\ {0 \preccurlyeq \hat{\Sigma} \preccurlyeq \Sigma} }} \,  \|\Sigma - \hat{\Sigma}\|_F^2 \nonumber \\
&=  \min_{\substack{ {\hat{\Sigma} \in \reals^{d \times d}} \\ {{\rm rank}(\hat{\Sigma}) = r} \\ {0 \preccurlyeq \hat{\Sigma} \preccurlyeq \Sigma} }} \,  \|\Sigma\|^2_F - \|\hat{\Sigma}\|^2_F + 2\Ip{\hat{\Sigma}}{\hat{\Sigma} - \Sigma}  \nonumber \\
&\leq  \min_{\substack{ {\hat{\Sigma} \in \reals^{d \times d}} \\ {{\rm rank}(\hat{\Sigma}) = r} \\ {0 \preccurlyeq \hat{\Sigma} \preccurlyeq \Sigma} }} \, \|\Sigma\|^2_F - \|\hat{\Sigma}\|^2_F \,. %
\end{align}
where we used
$\Ip{\hat{\Sigma}}{\hat{\Sigma} - \Sigma} 
= \Ip{\id}{\hat{\Sigma}^{1/2}(\hat{\Sigma} - \Sigma)\hat{\Sigma}^{1/2}}  %
= \sum_{i = 1}^d (\hat{\Sigma}^{1/2} e_i)^T (\hat{\Sigma} - \Sigma) (\hat{\Sigma}^{1/2} e_i) %
\leq 0$,
which follows from $\hat\Sigma \preccurlyeq \Sigma$. The minimum value of RHS above is achieved iff $\hat{\Sigma} =\Sigma_r$, since
\begin{align}
\|\Sigma - \Sigma_r \|_F^2 = \|\sum_{i = r+1}^d \sigma_i u_i u_i^T \|_F^2 = \sum_{i = r+1}^d \sigma_i^2 =  \sum_{i = 1}^d \sigma_i^2 -  \sum_{i = 1}^r \sigma_i^2
&= \|\Sigma\|^2_F - \|\Sigma_r\|^2_F\,.
\end{align}
and since LHS has a unique minima $\Sigma_r$ (Eckart–Young–Mirsky theorem), $\|\Sigma - \Sigma_r \|_F^2 < \|\Sigma - \hat{\Sigma}\|_F^2 \leq \|\Sigma\|^2_F - \|\hat{\Sigma}\|^2_F$ for any other $\hat{\Sigma} \neq \Sigma_r$. 

Therefore, $\max_{\substack{ {\hat{\Sigma} \in \reals^{d \times d}} \\ {{\rm rank}(\hat{\Sigma}) = r} \\ {0 \preccurlyeq \hat{\Sigma} \preccurlyeq \Sigma} }} \, \|\hat{\Sigma}\|^2_F$ is maximized only iff $\hat{\Sigma} =\Sigma_r$. This, along with the fact that $0 \preccurlyeq B_r B_r^T = \Sigma_r \preccurlyeq \Sigma$ if $B_r = \sum_{i=1}^r \sqrt{\sigma_i} u_i e_i^T \in \reals^{d \times r}$ implies that $\max_{\substack{{B \in \reals^{d \times r}} \\ {BB^T \preccurlyeq \Sigma}}} \,  \|BB^T\|_F^2$ is maximized iff $BB^T = \Sigma_r$. Therefore, by the existence of SVD, $B =  \sum_{i=1}^r \sqrt{\sigma_i} u_i v_i^T$, where ${v_i}_{i=1}^r$ is set of orthonormal vectors in $\reals^r$.

Finally, we show that the maximum of the divergence, $\max_{\substack{{G \in \mathcal{G}} \\ {X = G(C,Z) \sim \cN_{d}(0, \Sigma)}}} \frac1{4(r-1)} \sum_{\substack{i,j \in [r] \\ i \neq j}} \|\Sigma^{(i)} - \Sigma^{(j)}\|_F^2$, is achieved iff $B =  \sum_{i=1}^r \sqrt{\sigma_i} u_i e_{\pi(i)}^T$. First notice that $B=B_r$ satisfies this condition and $\Ip{b_r^{(i)}}{b_r^{(j)}} = \Ip{\sqrt{\sigma_i} u_i}{\sqrt{\sigma_j} u_j} = 0$, if $i \neq j$. Therefore $B_r$ is a maximizer for the divergence.

For any $i \neq j$, let $0 = \Ip{b^{(i)}}{b^{(j)}}$, then
\begin{align}
 0 = \Ip{b_r^{(i)}}{b_r^{(j)}} &= \Ip{\sum_{k=1}^r \sqrt{\sigma_k} u_k v_k^T e_i}{\sum_{k=1}^r \sqrt{\sigma_k} u_k v_k^T e_j} \nonumber \\
&= \sum_{k=1}^r  \Ip{\sqrt{\sigma_k} v_k^T e_i}{ \sqrt{\sigma_k} v_k^T e_j} \nonumber \\
&= e_i^T (\sum_{k=1}^r \sigma_k v_k v_k^T) e_j = e_i^T V_r e_j \,.
\end{align}
where we set $V_r = \sum_{k=1}^r \sigma_k v_k v_k^T$. Since $\{v_i\}_{i=1}^r$ is set of orthonormal vectors, $V_r$ is full-rank. Therefore, for any $\{a_{ij} \in \reals \}_{i,j=1}^r $, $(\sum_{j \neq i} a_{ij} e_j) ^T V_r e_i = 0$, which implies that $V_r e_i \perp {\rm span}(\{e_i\}_{j \neq i})$, which in turn implies that $\{e_i\}_{i=1}^r$ are the eigen vectors of $V_r$. Therefore $v_i = e_{\pi(i)}$ for some permutation $\pi: [r] \to [r]$.
\end{proof}

\input{oogan.tex}

}

==> experiment_lzn.tex <==
\section{Experiments}
\label{sec:exp}

We run experiments on a combination of synthetic datasets with pre-defined latent factors and real-world datasets.
The synthetic datasets enable us to numerically quantify disentanglement, thereby facilitating the comparison of protocols.
The real-world datasets provide only qualitative feedback, but show that our protocol works on more realistic data.\footnote{The code for all experiments is submitted with the supplementary materials.}

\subsection{Metrics}
\label{sec:metrics}
We measure both disentanglement and image quality to quantify the tradeoffs involved.  


\begin{table*}[h!]
	\begin{center}
	\begin{tabular}{| c | c | l | l |}
		\hline
	             & \textbf{Model}                                                                                                                                                               
	             & \begin{tabular}[c]{@{}l@{}} \textbf{Disentanglement} \\ (Kim \& Mnih) \end{tabular}                                
	             & \begin{tabular}[c]{@{}l@{}}			\textbf{Disentanglement}\\ (Eastwood \& Williams)\end{tabular}                              \\ \hline
			\textbf{VAE} 
			& \begin{tabular}[c]{@{}c@{}}VAE ($\beta=1.0$)\\ $\beta$-TCVAE ($\beta=4.0$)\\ HFVAE ($\beta=4.0, \gamma=3.0$)\\ CHyVAE \\ $\beta$-VAE ($\beta=4.0$)\\ FactorVAE*\end{tabular} 
			& \begin{tabular}[c]{@{}l@{}}$0.63 \pm 0.06$\\ 			$0.62 \pm0.07$\\ $0.63 \pm 0.08$\\ 0.77\\ 0.78\\ 0.82\end{tabular} 
			& \begin{tabular}[c]{@{}l@{}}$0.30 \pm 0.10$\\ $0.29 \pm 0.10$\\ $0.39 \pm 0.16$\\ \\ $0.41 \pm 0.11$ \\ $\boldsymbol{0.74 \pm 0.01}$ \end{tabular} \\ \hline
			\textbf{GAN} 
			& \begin{tabular}[c]{@{}c@{}}InfoGAN*\\ IB-GAN\\ InfoGAN (modified)*\\ InfoGAN-CR* (ours)\end{tabular}                                                                              			& \begin{tabular}[c]{@{}l@{}}$0.59 \pm 0.70$\\ $0.80 \pm 0.07$\\ $0.83 \pm 0.03$\\ 			$\boldsymbol{0.90 \pm 0.01}$\end{tabular}   
			& \begin{tabular}[c]{@{}l@{}}$0.41 \pm 0.05$\\ $0.67 \pm 0.07$\\ $0.56 \pm 0.03$\\ $\boldsymbol{0.74 \pm 0.01}$\end{tabular}    \\ \hline
	\end{tabular}
  	\end{center}
  	\caption{Comparisons of the disentanglement metric proposed in \cite{KM18} on the dSprite dataset. 
	A perfect disentanglement corresponds to a score of 1.0. 
	The proposed \gan achieves the highest  score, compared to 
	the best score reported in the literature for each 
	baseline from \cite{KM18,IBGAN,EWJ18,CHYVAE,LBL18}. 
	Asterisks denote experiments that we ran or confirmed ourselves. 
	InfoGAN (modified) is explained in Section \ref{sec:implementation}.} 
  	\label{tbl:comp}
\end{table*}

\paragraph{Disentanglement} We use the popular disentanglement metric proposed by \citet{KM18}. 
This metric is defined for datasets with known ground truth factors and is computed as follows. 
First, generate data points where the $i$th factor is fixed, but the other factors are varying uniformly at random, for a randomly-selected $i$. 
Pass each sample through the encoder, and normalize each resulting dimension by its empirical variance. 
Take the resulting dimension $j$ with the smallest variance. 
In a setting with perfect disentanglement, $j=i$, and the variance in the $j$th dimension would be 0.
Each sample's encoding generates a `vote' $j$; we take the majority vote as the final output of the classifier; if the classifier is correct, it should map to $i$. 
The disentanglement metric is the error rate of this classifier, taken over many independent trials of this procedure. 
In our experiment, for each fixed factor index $i$, we generate 100 groups of images, where each group has 100 images with the same value at the $i$th index. 

One challenge is computing the disentanglement metric for FactorVAE when trained with more latent codes $k$ than there are latent factors (let $z$ denote the true number of factors). 
For instance, \cite{KM18} uses $c\in \mathbb R^{10}$ for datasets with only five latent codes. 
To account for this, \cite{KM18} first removes all latent codes that have collapsed to the prior (i.e., $Q_{c_j|x}=P_{c_j}$); they then use the majority vote on the remaining factors.
However, this approach can artificially change the metric if the number of factors for which the posterior does not equal the prior does not equal $z$. 
Hence to measure the metric on FactorVAE (or more generally, cases where $k>z$), we first compute the $k \times z$ metric matrix, find the maximum value of each row. 
We then take the top $z$ among the $k$ maximum row values, and sum them up.


We additionally compute the (less common) disentanglement metric of \cite{EW18}. 
This metric first requires an estimate of the disentangled code $\tilde c$ from the generated samples, for which we use our encoder.
Next, we train a regressor $f$ to predict $c$ from $\tilde c$, so $\hat c = f(\tilde c)$. 
These regressors must also provide a matrix of relative importance $R$, such that $R_{ij}$ denotes the relative importance of $\tilde c_i$ in predicting $\hat c_j$.
Because of this requirement, Eastwood and Williams propose using regressors that provide importance scores, such as LASSO and random forests.
These restrictions limit the generality of the metric; nonetheless, we include it for completeness.
Given the regression $f$, disentanglement is computed for the $i$th latent code as 
$
D_i = (1-H(W_{i.}))
$
where $H(\cdot)$ is the entropy of $W_{i.}$, and $W_{ij}=R_{ij}/\sum_{\tilde k=0}^k R_{i\tilde k}$.
The final disentanglement score is $D = \frac{1}{k} \sum_i D_i$.



\paragraph{Data Quality}
We measure data quality with three metrics: Inception score, KL divergence, and classifier confidence. 
\textit{Inception score} was first proposed in \cite{SGZ16} for labelled data, and is  computed as $\exp(\E_x d_{\rm KL}(p(y|\boldsymbol x) || p(y)))$, where 
$d_{\rm KL}$ denotes the Kullback-Liebler divergence of two distributions. 
The distribution $p(y|\boldsymbol x)$ was originally designed to be used with the Inception network \cite{SVI16}, but we instead use a pre-trained classifier for the dataset at hand. 
Notice that this metric does not require any information about the disentangled representation of a sample. 
Inception score is widely used in the GAN literature to evaluate data quality. 
We also describe more nuanced measures of image quality in Appendix \ref{app:metrics}, and measure them on our datasets.



\subsection{dSprites Dataset} 

We begin with the synthetic dSprites dataset \cite{dSprites}, which is commonly used to numerically compare disentangling methods. 
The dataset consists of 737,280 binary 64 $\times$ 64 images of 2D shapes generated from five ground truth independent latent factors: color, shape, scale, rotation, x and y position. 
All  combinations of latent factors are present in the dataset; Figure \ref{fig:dsprites} shows example images.

\begin{figure}[H]
	\centering
	\includegraphics[width=0.8in]{figures/sprites}
	\caption{Example images from the dSprites dataset.}
	\label{fig:dsprites}
\end{figure}

Figure \ref{fig:latenttraversal} illustrates the latent traversal for \gannosp.
To generate this figure, we fix all latent factors except one $c_i$, and vary $c_i$ from -1 to 1 in evenly-spaced intervals. 
We observe that each of the five empirically-learned factors captures one of the true underlying factors, and the traversals span the full range of possibilities for each hidden factor.




We compute and/or reproduce disentanglement metrics for a number of protocols in Table \ref{tbl:comp}. 
In this table, all algorithms with an asterisk were either run or independently confirmed by us.
We describe the architecture and implementation of all baselines and \gan in Section \ref{sec:implementation} and Appendix \ref{app:implementation}.
For the metric of \cite{KM18}, Table \ref{tbl:comp} shows that the baseline disentanglement of InfoGAN can be substantially boosted through better training, from 0.59 to 0.83.
Contrastive regularization provides an additional gain, bringing the disentanglement metric of \gan up to 0.90, higher than any of the baselines from the VAE or GAN literature. 
For the metric of \cite{EW18}, we find similar trends, except FactorVAE is tied with \gan for the best score.  



\subsubsection{Implementation details}
\label{sec:implementation}
We implemented both FactorVAE and InfoGAN  using the architectures described in \cite{KM18}.
For completeness, we describe both architectures in detail in Appendix \ref{app:implementation}.
Although InfoGAN exhibits a reported disentanglement score of $0.59 \pm 0.70$ in \cite{KM18},
we find that InfoGAN can exhibit substantially higher disentanglement scores ($0.83 \pm 0.03$) through some basic changes to the architecture and loss function. 
In particular, in accordance with \cite{MKKY18}, we changed the loss function from Wasserstein GAN to the traditional JSD loss. 
We also changed the generator's Adam learning rate to $0.001$ and the InfoGAN and CR discriminators learning rates to $0.002$;
we used 5 continuous input codes, whereas \cite{KM18} reported using four continuous codes and one discrete one.
We also used batch normalization in the generator, and spectral normalization in the discriminator. 
Finally, we used InfoGAN regularizer $\lambda = 0.05$, and for \gannosp, we used contrastive regularizer $\alpha=2.0$.
The effects of these changes are shown in the line `InfoGAN (modified)' in Table \ref{tbl:comp}.
For FactorVAE, we used the architecture of \cite{KM18}, which uses $k=10$ latent codes in their architecture. 
To compute disentanglement, we use the technique described in Section \ref{sec:metrics}.











\subsubsection{Design Space Exploration}

\paragraph{Parameters.}
We start by showing the effect of varying \gannosp's parameters: the InfoGAN regularizer $\lambda$ and the contrastive regularizer $\alpha$.
In particular, we are interested in understanding how these parameters trade off disentanglement with image quality. 
To this end, we vary both parameters and compute both the disentanglement metric of \cite{KM18} and inception score. 
Since inception scores can only be computed for labelled, categorical data, we compute it over the `shape' latent factor, which has three options: heart, square, or oval. 
Figure \ref{fig:varying_alpha} shows the resulting trends, both for  \gannosp and for modified InfoGAN (which is a special case with $\alpha=0$).
For \gannosp, we set $\lambda \in \{0.05, 0.2, 2.0\}$ and take $\alpha \in \{0,1,2,4,8\}$.
The size of each point in Figure \ref{fig:varying_alpha} corresponds to the value of $\alpha$, which we explicitly label for $\lambda=0.05$ (blue triangles). 
Each data point is averaged over 11 runs.
As we increase the contrastive regularizer, inception score decreases, whereas disentanglement improves up to a point, and then decreases.
Notably, using contrastive regularizer $\alpha=1$ or $\alpha=2$ seems to incur small reductions in inception score for a significant boost in disentanglement.
To better understand these results, we generated similar plots using more nuanced image quality metrics. 
These metrics and plots are included in Appendices \ref{app:metrics} and \ref{app:parameters}.

\begin{figure}[h]
	\includegraphics[width=3in]{figures/varying_alpha}
	\put(-135,-5){Inception Score}
	\put(-62,92){$\alpha=0$}
	\put(-72,116){$\alpha=1$}
	\put(-95,134){$\alpha=2$}
	\put(-150,114){$\alpha=4$}
	\put(-175,103){$\alpha=8$}
	\put(-220,50){\rotatebox{90}{Disentanglement}}
	\caption{ Achievable (inception score, disentanglement) pairs for \gannosp, where disentanglement is measured as in \cite{KM18}. We vary the contrastive regularizer $\alpha$ and the InfoGAN regularizer $\lambda$.
	The size of each point denotes $\alpha \in \{0,1,2,4,8\}$, in order of increasing size; we have explicitly labelled this for $\lambda=0.05$ (blue triangles). 
	}
	\label{fig:varying_alpha}
\end{figure}



\paragraph{Progressive Training.}
One key aspect of contrastive regularization is its progressive reduction of the contrastive gap during training. 
In this section, we show the importance of progressive training by comparing it to regularization for a fixed gap. 
Figure \ref{fig:progressive} shows the disentangling metric of \cite{KM18} as a function of batch number. 
For the `progressive  training' curve, we use a contrastive gap of 1.9 for 120,000 batches, and then introduce a (more aggressive) gap of 0. 
For the `no progressive training' curves, we use gap size of 0 or 1.9 for all 230,400 batches. 
All curves use an InfoGAN regularizer $\lambda = 0.7$ and a CR weight $\alpha=1.0$.
Notice that the results in Table \ref{tbl:comp} were computed for a different value of $\lambda$, which explains why Figure \ref{fig:progressive} achieves lower disentanglement scores.
The progressive training curve is averaged over 10 runs, whereas the `no progressive training' curves are averaged over 21 runs. 
We observe that progressive training helps the disentanglement metric grow faster than either of the settings without progressive training. 
We also tried a smooth progressive training schedule (e.g. smoothly decreasing the contrastive gap), but found this to destabilize training. 

\begin{figure}[t]
	\centering
	\includegraphics[width=2.9in]{figures/prog_training2}
	\put(-130,-7){Batch number}
	\put(-215,50){\rotatebox{90}{Disentanglement}}
	\caption{Reducing the contrastive gap  from  1.9 to 0 during training gives better disentanglement scores than  either fixed gap.
	}
	\label{fig:progressive}
\end{figure}



\paragraph{Objective Function.}
We claim that contrastive regularization is specifically tailored to work well with GAN architectures. 
Similarly, we claim that total correlation regularization of FactorVAE is specifically tailored for VAE. 
To test this hypothesis, we have applied contrastive regularization (CR) to FactorVAE and total correlation (TC) regularization to InfoGAN-CR.
Figure \ref{fig:vae_vs_gan} shows the disentanglement metric of each as a function of batch numbers. 
For FactorVAE, we introduce CR regularization of $\alpha = 20$ at batch 300,000. 
Note that the metric does not change perceptibly after adding CR. 
For InfoGAN-CR, we ran one set of trials with TC regularization from the beginning (red curve) and one set of trials without TC regularization (green curve). 
We use InfoGAN regularizer $\lambda = 0.7$ and TC coefficient $\beta = 1$ for the former.
Notice that \gan has a lower disentanglement score than FactorVAE in this plot because we did not use the optimal $\lambda$ for this dataset; 
this sensitivity is a weakness of \gannosp.
In Figure \ref{fig:vae_vs_gan}, we observe that TC regularization actually reduces disentanglement compared to InfoGAN-CR without TC.
The jumps in disentanglement for the \gan curves are due to progressive training; we change the contrastive gap from 1.9 to 0.0 at batch 120,000.
The red line (\gan + TC) is averaged over 4 runs, the blue line (FactorVAE + CR) over 2 runs, and the green line (\gannosp) over ten.
These results support (but do not prove) our hypothesis that CR is better-suited to GAN architectures, whereas TC is better-suited to VAE architectures. 
To further confirm  this intuition, we show that disentanglement appears negatively correlated with a measure of total correlation in Appendix \ref{app:tc}.

\begin{figure}[t]
	\centering
	\includegraphics[width=2.9in]{figures/vae_vs_gan}
	\put(-125,-7){Batch number}
	\put(-218,50){\rotatebox{90}{Disentanglement}}
	\caption{Adding TC regularization to InfoGAN-CR does not improve disentanglement; neither does adding CR to FactorVAE.
	}
	\label{fig:vae_vs_gan}
\end{figure}
































\subsection{Teapots Dataset}
We confirm  our results from the dSprites dataset on the teapots dataset proposed in \cite{EW18}. 
This dataset contains images of teapots in various orientations and colors, generated by the renderer in \cite{MW16}. 
These images have five latent factors: color (red, blue, and green channels), rotation (vertical), and rotation (lateral); each is represented as continuous in $[-1,1]$. Colors are randomly drawn from $[0,1]$. Rotation (vertical) is randomly drawn from $[0,\pi/2]$. Rotation (lateral) is randomly drawn from $[0, 2\pi]$.
We generated a dataset of 200,000 such images with each combination of latent factors represented. 

Table \ref{tbl:teapot} shows the disentanglement scores of FactorVAE and InfoGAN compared to \gannosp;
again, we observe that \gan achieves a higher disentanglement score than the other baselines, 
and contrastive regularization increases the metric compared to modified InfoGAN. 
Since the teapots dataset does not have a natural  notion of classes, we do not compute inception score for this dataset. 
However, we include latent traversal images for the dataset in Appendix \ref{app:teapots}, and note that the images generated by \gan appear sharper than those generated by FactorVAE.
We also include plots showing the evolution of the disentanglement metric over the training period for all baselines in Appendix \ref{app:teapots}.


\subsubsection{Implementation Details}
\label{sec:teapots_impl}

For the teapots dataset, we used an identical architecture to the dSprites dataset for InfoGAN and FactorVAE. 
For \gannosp, the CR discriminator architecture changed slightly and is listed in Table \ref{tab:cr_teapots_arch}.
As with dSprites, FactorVAE used 10 latent codes, so we again chose the best five to compute the disentanglement metric of \cite{KM18}.

\begin{table}[]
\begin{tabular}{|l|l|}
\hline
\textbf{Scheme}                          & \begin{tabular}[c]{@{}l@{}}\textbf{Disentanglement}\\ (Kim \& Mnih)\end{tabular} \\ \hline
FactorVAE ($\beta=1$)                    &                        $0.65 \pm 0.04$                                                          \\ \hline
FactorVAE ($\beta=10$)                   &                        $0.62 \pm 0.03$                                                         \\ \hline
FactorVAE ($\beta=20$)                   &                         $0.67 \pm 0.04$                                                         \\ \hline
FactorVAE ($\beta=40$)                   &                         $0.79 \pm 0.03$                                                         \\ \hline
InfoGAN (modified, $\lambda=0.2$)        &            $0.76 \pm 0.06$                                                                      \\ \hline
InfoGAN-CR ($\lambda=0.2$, $\alpha=1.0$) &   $\boldsymbol{0.86 \pm 0.03}$                                                                                \\ \hline
\end{tabular} 
\caption{Disentanglement metrics for teapot dataset.}
\label{tbl:teapot}
\end{table}


\subsection{CelebA Dataset}
Finally, we tested \gan on the CelebA dataset to observe its performance on real-world data. 
CelebA is a dataset of 202599 facial images from celebrities. 
Since these images do not have known latent factors or labelled categories, we cannot compute the disentanglement metric or inception score. 
We therefore evaluate this dataset qualitatively, by producing latent traversals. 
Figure \ref{fig:celeba_traversal} shows such a traversal for \gannosp, suggesting that \gan is able to learn latent factors like hair color, rotation, lighting, background, and hair style.
Details of our architecture are included in Appendix \ref{app:celeba}.

\begin{figure}[t]
	\includegraphics[width=2.9in]{figures/latent_celeba}
	\put(0,65){Hair color}
	\put(0,50){Rotation}
	\put(0,35){Lighting}
	\put(0,20){Background}
	\put(0,5){Bangs}
	\caption{Adding TC regularization to InfoGAN-CR does not improve disentanglement; neither does adding CR to FactorVAE.
	}
	\label{fig:celeba_traversal}
\end{figure}

\section{Exploring Choices CR}
In the design of CR, there are 4 choices, based on how the two input images are generated, when assuming gap is always zero:
\begin{enumerate}
	\item Same noise variables, and same latent codes except one
	\item Same noise variables, and random latent codes except one
	\item Random noise variables, and same latent codes except one
	\item Random noise variables, and random latent codes except one
\end{enumerate}

We tried all four settings in MNIST dataset, using architecture in \cite{CDH16}, with 1 10-category latent codes, 2 continuous latent codes, and 62 noise variables. We had 8 runs for each setting, and visually inspect whether it correctly disentangle digit, rotation, and width. The disentanglement successful rate are recorded in table \ref{tbl:mnist}.

\begin{table}
	\begin{tabular}{|l|l|}
		Choice & Rate of Successful Disentanglement\\\hline
		1 & 5/8\\\hline
		2 & 8/8\\\hline
		3 & 2/8\\\hline
		4 & 6/8\\\hline
	\end{tabular}
	\caption{Rate of successful disentanglement using four choices of CR}	\label{tbl:mnist}
\end{table}

Based on this result, we choose to use option 2 as our starting point of designing CR.
